Texture Learning Domain Randomization for Domain Generalized Segmentation

Deep Neural Networks (DNNs)-based semantic segmentation models trained on a source domain often struggle to generalize to unseen target domains, i.e., a domain gap problem. Texture often contributes to the domain gap, making DNNs vulnerable to domain shift because they are prone to be texture-biased. Existing Domain Generalized Semantic Segmentation (DGSS) methods have alleviated the domain gap problem by guiding models to prioritize shape over texture. On the other hand, shape and texture are two prominent and complementary cues in semantic segmentation. This paper argues that leveraging texture is crucial for improving performance in DGSS. Specifically, we propose a novel framework, coined Texture Learning Domain Randomization (TLDR). TLDR includes two novel losses to effectively enhance texture learning in DGSS: (1) a texture regularization loss to prevent overfitting to source domain textures by using texture features from an ImageNet pre-trained model and (2) a texture generalization loss that utilizes random style images to learn diverse texture representations in a self-supervised manner. Extensive experimental results demonstrate the superiority of the proposed TLDR; e.g., TLDR achieves 46.5 mIoU on GTA-to-Cityscapes using ResNet-50, which improves the prior state-of-the-art method by 1.9 mIoU. The source code is available at https://github.com/ssssshwan/TLDR.

==> ablation_lr.tex <==
\begin{tabular}{llcccc}
\hline
  & Case                                          & C     & B     & M     & S     \\ \hline
\rowcolor[HTML]{E6E6E6} 
1 & w/ Warmup                                     & 00.00 & 00.00 & 00.00 & 00.00 \\
2 & w/o Warmup                                    & 00.00 & 00.00 & 00.00 & 00.00 \\ \hline
\rowcolor[HTML]{E6E6E6} 
3 & ${lr}_{enc}$$=$${lr}_{dec}\ / 10$ & 00.00 & 00.00 & 00.00 & 00.00 \\
4 & ${lr}_{enc}$$=$${lr}_{dec}$                  & 00.00 & 00.00 & 00.00 & 00.00 \\ \hline
\end{tabular}

==> classwise.tex <==
\begin{tabular}{lllll|ccccccccccccccccccc|c}
\hline
 &
  $L_{orig}$ &
  $L_{styl}$ &
  $L_{tr}$ &
  $L_{tg}$ &
  Road &
  Sidew. &
  Build. &
  Wall &
  Fence &
  Pole &
  Tr.light &
  Sign &
  Veget. &
  Terrain &
  Sky &
  Person &
  Rider &
  Car &
  Truck &
  Bus &
  Train &
  M.bike &
  Bike &
  mIoU \\ \hline
1 &
  $\checkmark$ &
  - &
  - &
  - &
  52.9 &
  33.7 &
  52.6 &
  15.5 &
  27.6 &
  30.7 &
  49.0 &
  24.7 &
  83.8 &
  23.8 &
  37.6 &
  67.2 &
  23.4 &
  72.8 &
  17.0 &
  21.9 &
  2.0 &
  17.7 &
  32.5 &
  36.1 \\
2 &
  - &
  $\checkmark$ &
  - &
  - &
  78.9 &
  40.5 &
  72.0 &
  18.6 &
  15.1 &
  32.4 &
  26.8 &
  30.2 &
  82.4 &
  28.5 &
  72.7 &
  60.9 &
  30.5 &
  69.6 &
  26.0 &
  30.7 &
  2.5 &
  12.6 &
  19.2 &
  39.5 \\
3 &
  $\checkmark$ &
  $\checkmark$ &
  - &
  - &
  72.9 &
  37.7 &
  71.3 &
  17.7 &
  21.2 &
  38.2 &
  48.2 &
  35.3 &
  86.1 &
  24.9 &
  72.2 &
  68.7 &
  30.4 &
  85.2 &
  21.8 &
  35.5 &
  4.2 &
  28.1 &
  29.2 &
  43.6 \\
4 &
  $\checkmark$ &
  $\checkmark$ &
  $\checkmark$ &
  - &
  82.7 &
  41.2 &
  78.6 &
  26.6 &
  27.5 &
  39.5 &
  45.2 &
  34.8 &
  86.8 &
  27.7 &
  71.0 &
  68.7 &
  29.9 &
  83.6 &
  37.6 &
  44.0 &
  1.6 &
  29.1 &
  34.2 &
  46.8 \\
5 &
  $\checkmark$ &
  $\checkmark$ &
  - &
  $\checkmark$ &
  79.6 &
  40.4 &
  76.2 &
  28.6 &
  25.0 &
  37.3 &
  49.2 &
  34.7 &
  86.6 &
  27.3 &
  79.5 &
  68.9 &
  35.8 &
  78.4 &
  32.6 &
  34.9 &
  9.9 &
  27.0 &
  28.9 &
  46.4 \\
 6 &
  $\checkmark$ &
  $\checkmark$ &
  $\checkmark$ &
  $\checkmark$ &
  82.3 &
  40.4 &
  81.2 &
  26.1 &
  26.5 &
  37.3 &
  49.4 &
  35.0 &
  85.6 &
  29.4 &
  82.2 &
  68.7 &
  32.8 &
  84.1 &
  39.5 &
  40.4 &
  9.1 &
  23.5 &
  33.0 &
  47.8 \\ \hline
\end{tabular}

==> comparison.tex <==
\begin{tabular}{lccccclcccclcccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Method}} &
  \multirow{2}{*}{Backbone} &
  \multicolumn{4}{c}{Train on GTA5 (G)} &
   &
  \multicolumn{4}{c}{Train in SYNTHIA (S)} &
   &
  \multicolumn{4}{c}{Train on Cityscapes (C)} \\ \cline{3-6} \cline{8-11} \cline{13-16} 
\multicolumn{1}{c}{} &
   &
  $\rightarrow$C &
  $\rightarrow$B &
  $\rightarrow$M &
  $\rightarrow$S &
   &
  $\rightarrow$C &
  $\rightarrow$B &
  $\rightarrow$M &
  $\rightarrow$G &
   &
  $\rightarrow$B &
  $\rightarrow$M &
  $\rightarrow$G &
  $\rightarrow$S \\ \hline
IBN-Net \cite{pan2018two} &
\multirow{5}{*}{ResNet-50} &
  33.8 &
  32.3 &
  37.8 &
  27.9 &
   &
  32.0 &
  30.6 &
  32.2 &
  26.9 &
   &
  48.6 &
  57.0 &
  45.1 &
  26.1 \\
DRPC \cite{yue2019domain} &
   &
  37.4 &
  32.1 &
  34.1 &
  28.1 &
   &
  35.6 &
  31.5 &
  32.7 &
  28.8 &
   &
  49.9 &
  56.3 &
  45.6 &
  26.6 \\
RobustNet \cite{choi2021robustnet} &
   &
  36.6 &
  35.2 &
  40.3 &
  28.3 &
   &
  35.8 &
  31.6 &
  30.8 &
  27.7 &
   &
  50.7 &
  58.6 &
  45.0 &
  26.2 \\
SAN-SAW \cite{peng2022semantic} &
   &
  $\underline{39.8}$ &
  $\underline{37.3}$ &
  $\underline{41.9}$ &
  $\underline{30.8}$ &
   &
  $\underline{38.9}$ &
  $\textbf{35.2}$ &
  $\underline{34.5}$ &
  $\underline{29.2}$ &
   &
  $\underline{53.0}$ &
  $\underline{59.8}$ &
  $\underline{47.3}$ &
  $\underline{28.3}$ \\
Ours (TLDR) &
   &
  $\textbf{46.7}$ &
  $\textbf{42.7}$ &
  $\textbf{45.1}$ &
  $\textbf{37.1}$ &
   &
  $\textbf{40.5}$ &
  $\underline{34.9}$ &
  $\textbf{37.4}$ &
  $\textbf{36.4}$ &
   &
  00.0 &
  00.0 &
  00.0 &
  00.0 \\ \hline
IBN-Net \cite{pan2018two} &
  \multirow{5}{*}{ResNet-101} &
  37.4 &
  38.3 &
  38.3 &
  28.7 &
   &
  34.2 &
  36.6 &
  36.2 &
  28.2 &
   &
  50.2 &
  58.4 &
  46.3 &
  27.6 \\
DRPC \cite{yue2019domain} &
   &
  42.5 &
  38.7 &
  38.1 &
  29.7 &
   &
  37.6 &
  34.3 &
  34.1 &
  29.2 &
   &
  51.5 &
  58.6 &
  46.9 &
  29.0 \\
RobustNet \cite{choi2021robustnet} &
   &
  42.9 &
  38.5 &
  39.1 &
  29.6 &
   &
  37.2 &
  34.0 &
  35.9 &
  29.0 &
   &
  51.0 &
  59.7 &
  46.3 &
  28.4 \\
SAN-SAW \cite{peng2022semantic} &
   &
  $\underline{45.3}$ &
  $\underline{41.2}$ &
  $\underline{40.8}$ &
  $\underline{31.8}$ &
   &
  $\underline{40.9}$ &
  $\underline{35.0}$ &
  $\underline{37.3}$ &
  $\underline{30.8}$ &
   &
  $\underline{54.7}$ &
  $\underline{61.3}$ &
  $\underline{48.8}$ &
  $\underline{30.2}$ \\
Ours (TLDR) &
   &
  $\textbf{47.8}$ &
  $\textbf{44.6}$ &
  $\textbf{48.4}$ &
  $\textbf{39.6}$ &
   &
  $\textbf{42.8}$ &
  $\textbf{36.3}$ &
  $\textbf{38.9}$ &
  $\textbf{39.0}$ &
   &
  00.0 &
  00.0 &
  00.0 &
  00.0 \\ \hline
\end{tabular}

==> shape.tex <==
\begin{tabular}{llcccc}
\hline
  & Method      & SC    & SB    & SM    & SS    \\ \hline
1 & Baseline & 2.60  & 1.46  & 1.87  & 3.17  \\
2 & DR       & 26.90 & 24.78 & 24.53 & 23.40 \\
3 & TLDR     & 29.36 & 30.30 & 31.08 & 24.06 \\ \hline
\end{tabular}
